Breakpoint based online anomaly detection

The goal of anomaly detection is to identify observations that are generated by a distribution that differs from the reference distribution that qualifies normal behavior. When examining a time series, the reference distribution may evolve over time. The anomaly detector must therefore be able to adapt to such changes. In the online context, it is particularly difficult to adapt to abrupt and unpredictable changes. Our solution to this problem is based on the detection of breakpoints in order to adapt in real time to the new reference behavior of the series and to increase the accuracy of the anomaly detection. This solution also provides a control of the False Discovery Rate by extending methods developed for stationary series.

==> mes-macros2.tex <==
\newcommand{\testtexmf}{success}


% Math operators
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}



% new columns types
\newcolumntype{R}[1]{>{\raggedleft\arraybackslash }b{#1}}
\newcolumntype{L}[1]{>{\raggedright\arraybackslash }b{#1}}
\newcolumntype{C}[1]{>{\centering\arraybackslash }b{#1}}

% new theorems

\theoremstyle{plain}
\newtheorem{definition}{Definition}
\newtheorem{proposition}{Proposition}
%\theoremstyle{plain}
%\newtheorem{mydef}{Definition}
\newtheorem{theorem}{Theorem}
%\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}[theorem]
\newtheorem{corollary}{Corollary}

%glossaire
\newacronym{kcp}{KCP}{Kernel Change Point}
\newacronym{kde}{KDE}{Kernel Density Estimator}
\newacronym{ml}{ML}{Machine Learning}
\newacronym{arma}{ARMA}{Auto Regressive Moving Average}
\newacronym{rkhs}{RKHS}{Reproducing Kernel Hilbert Space}
\newacronym{momkde}{MOM-KDE}{Medians-of-means Kernel Density Estimator}
\newacronym{bh}{BH}{Benjamini-Hochberg}
\newacronym{fdr}{FDR}{False Datection Rate}
\newacronym{fnr}{FNR}{False Negative Rate}
\newacronym{fpr}{FPR}{False Positive Rate}
\newacronym{it}{IT}{Information Technology}


% commands
\newcommand{\X}{\mathcal{X}}
%\newcommand{\todo}[1]{\textcolor{red}{#1}}
\newcommand{\todo}[1]{\textcolor{red}{#1}}
\newcommand{\wrap}[1]{\raisebox{.5pt}{\textcircled{\raisebox{-.9pt} {#1}}}}
\newcommand{\done}[1]{\textcolor{blue}{#1}}
\newcommand{\R}{\mathbb{R}}

\newcommand{\1}{\mathds{1}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\II}{\mathbf{1}}
\newcommand{\Hzero}{\mathcal{H}_0}
\newcommand{\Hone}{\mathcal{H}_1}
\newcommand{\alterdistrib}{\mathcal{P}_{1}}
\newcommand{\refdistrib}{\ensuremath{\mathcal{P}_{0}}}
\newcommand{\winsize}{m}
\newcommand{\calset}{\lbrace x_1, ... ,x_n \rbrace}
\newcommand{\trainset}{z_{1}^{\ell}}
\newcommand{\pv}{\ensuremath{p\mbox{-value}}}

\newcommand{\undertrain}[1]{\underbrace{#1}_{\mbox{train}}}
\newcommand{\undercal}[1]{\underbrace{#1}_{\mbox{calibration}}}
\newcommand{\undertest}[1]{\underbrace{#1}_{\mbox{test}}}


\newcommand{\hsp}{\hspace{20pt}}
\newcommand{\HRule}{\rule{\linewidth}{0.5mm}}

% Notations
%% Time series
\newcommand{\obs}{\ensuremath{x}}
\newcommand{\stopro}{\ensuremath{X}}

%% p-valeurs
\newcommand{\pvalue}{\ensuremath{G}}
\newcommand{\hpvalue}{\hat G}
\newcommand{\density}{p}
\newcommand{\hdensity}{\hat p}

%% KCP
\newcommand{\riskkcp}{R}
\newcommand{\nbs}{D}
\newcommand{\kernel}{K}
\newcommand{\seg}{\ensuremath{\tau}}

%% Forecasting
\newcommand{\backcast}{}
%{\tiny }
\newcommand{\forecast}{}

%% KDE
\newcommand\ised[1]{\ensuremath{ISE_d(#1)}}
\newcommand\isetsf[1]{\ensuremath{ISE^t_{sf}(#1)}}
\newcommand\mised[1]{\ensuremath{ISE_d(#1)}}
\newcommand\mistsf[1]{\ensuremath{ISE^t_{sf}(#1)}}

%% Confidence score
\newcommand{\V}{V}
\newcommand{\W}{W}

%% Anomal==



%% Edition
\newcommand{\blank}{\textcolor{red}{...}}
